High-throughput Execution of Hierarchical Analysis Pipelines on Hybrid Cluster Platforms

We propose, implement, and experimentally evaluate a runtime middleware to support high-throughput execution on hybrid cluster machines of large-scale analysis applications. A hybrid cluster machine consists of computation nodes which have multiple CPUs and general purpose graphics processing units (GPUs). Our work targets scientific analysis applications in which datasets are processed in application-specific data chunks, and the processing of a data chunk is expressed as a hierarchical pipeline of operations. The proposed middleware system combines a bag-of-tasks style execution with coarse-grain dataflow execution. Data chunks and associated data processing pipelines are scheduled across cluster nodes using a demand driven approach, while within a node operations in a given pipeline instance are scheduled across CPUs and GPUs. The runtime system implements several optimizations, including performance aware task scheduling, architecture aware process placement, data locality conscious task assignment, and data prefetching and asynchronous data copy, to maximize utilization of the aggregate computing power of CPUs and GPUs and minimize data copy overheads. The application and performance benefits of the runtime middleware are demonstrated using an image analysis application, which is employed in a brain cancer study, on a state-of-the-art hybrid cluster in which each node has two 6-core CPUs and three GPUs. Our results show that implementing and scheduling application data processing as a set of fine-grain operations provide more opportunities for runtime optimizations and attain better performance than a coarser-grain, monolithic implementation. The proposed runtime system can achieve high-throughput processing of large datasets - we were able to process an image dataset consisting of 36,848 4Kx4K-pixel image tiles at about 150 tiles/second rate on 100 nodes.

==> learning.tex <==
\section{Learning to Schedule}

In our work, we have so far asked the programmer to provides us with
information about the expected performance (speedup) of tasks when executed in
the GPU.  The idea here is to start working towards an automation of the
process learning the performance of application (stages of the application),
and use this information to automatically schedule the application in CPU-GPU
environments.

A few works have started addressing this problem on the context of modeling and
estimation of GPU application's performance, most of them using history based
strategy based on application
profiling~\cite{Augonnet:2009:ACP:1884795.1884805,gregg10contention,5645393,Jimenez:2008:PRC:1505816.1505822,Kicherer:2011:CFM:1944862.1944883}.
Most of these works, however, fail miserably to provide a generic approach, and
are very simplistic though they already show that doing such a profiling based
performance estimation is promising. A related interesting work for
multicores CPUs only is~\cite{LUO:2009:INRIA-00436034:1}, where the authors
take advantage of profile history to estimate the set of optimizations that
would result into the best performance for an application. In my understanding,
we could leverage some of their propositions in our work. Moreover, there is
also some work on performance modeling~\cite{1138092,1498789} which states that
computing relative performance among devices (different processors or disks,
etc) is easier than trying to estimate execution times. This is good news once
our scheduling policies are based on speedups. Another good news is that the
accuracy of the speedup estimates is not critical as long as the order of tasks
is not affected, as we stated for IPDPS. Also, a estimation that separates
tasks with small and large speedups should be enough to achieve good
performance.


To accomplish this task we will need the following components.

\begin{itemize}
	\item Knowledge Database: to store performance data collected;

	\item Performance fitting algorithms: to estimate performance from the history data stored at the Knowledge database;

	\item Automated task grouping: is one of the features that could be derived from this knowledge.
\end{itemize}





==> model.tex <==
\section{Analytical Performance Model}
\label{sec:model}
%
We present an analytical model to assess the performance of the scheduling and
optimizations proposed in this work. The main intention of this model is to
provide a set of tools that could be used to estimate the performance impact of
the proposed optimizations for a given set of tasks, which presumably comprise
a candidate application for implementation in our execution model, without
having to port the application to our system. 

The task scheduling problem in our work is dynamic in the sense that tasks may
be created during the computation, at timestamps unknown prior to the
execution. Thus, off-line scheduling is not possible and proper mapping
decisions must be carried out on-the-fly as tasks become available. The
analytical model constructed here is mostly common for all proposed scheduling
policies, which only differ in the final decision regarding to what task is
chosen for execution at each mapping time.

Let $T$ be the set of all tasks $w_i$, $1 \le i \le m$, computed by an
application during the execution, each of them created at a timestamp $c_i$ not
known prior to execution.  Assume that there is no preemption in a task
execution; each task is assigned to a single heterogeneous processor $p_j \in
p_1\dots p_n$; and, the estimated execution time of a given task $w_i$ using
processor $p_j$ is denoted as $e_{ij}$. Further, let $T^t$ be the set of tasks
created before or on timestamp $t$, which have not been scheduled for
execution.  The subset of tasks mapped to a given processor $p_j$ on or before
time $t$ is expressed as $PT_j^t$, the schedule for all processor at time $t$
as $PT^t$, and $idle_{ij}$ is the idle time elapsed between $w_i$ start time and the
end of the last task assigned to processor $p_j$.  Notice that $idle_{ij}$ may
represent several aspects as scheduling overhead, data transfer times required
to start a task, insufficient parallelism, or it could be also ignored for
simplified analysis. Further, $F(PT^t_j)$, the predicted finish time of machine
$j$ for tasks assigned on or before time $t$ may be calculated as:

\begin{equation}
F(PT^t_j) = \sum_{k \in PT_j^t} (e_{kj} + idle_{kj})
\end{equation}

In our approach, the mapping of tasks to processors is demand-driven and a
single task is assigned to a processor whenever at least one processor is
available ($\tau(PT^t) = \min_{1\le j \le n} F(PT^t_j)$), and there are tasks to be
scheduled ($T^t \neq \emptyset$). Additionally, the next non-empty set of
tasks on or after timestamp $t$ is $\zeta(t)$:

\begin{equation}
  \zeta(t) = \left\{ 
  \begin{array}{l l}
    t 		& \quad \text{if $T^t \neq \emptyset$}\\
    min_{1\le i\le m}(c_i\ |\ c_i > t) 	& \quad \text{otherwise}\\
  \end{array} \right.
\end{equation}

Thus, the next mapping time on or after a given timestamp $t$ may be calculated
as $\beta(t) = max(\tau(PT^t), \zeta(t))$. The processor to receive the next
task at a given mapping time $t'=\beta(t)$ is that processor with smallest predicted
finish time at timestamp $t'$ ($\phi(t') = \underset{1 \le j \le
n}{\operatorname{argmin}}\ F(PT^{t'}_j)$). Further, we define the function
$\vartheta(t)$ that calculates the mapping of a single task at time $t$:

\begin{equation}
\vartheta(t) = \beta(\tau(PT_{\phi(t)}^t \leftarrow select(T^{t}, POLICY)))
\label{eq:mapping}
\end{equation}

%\begin{equation}
%\vartheta(t) = \beta(\tau(PT_{\phi(\beta(t))} \leftarrow select(T^{\beta(t)}, POLICY)))
%\label{eq:mapping}
%\end{equation}

The $\vartheta(t)$ first calculates the set of tasks ready to execute at the
mapping time $t$ ($T^{t}$), selects one task according to the scheduling policy
chosen, e.g. FCFS or PRIORITY, and assigns that task to the processor with
minimum finish time at time $t$ ($\phi(t)$). After the mapping is performed, the
timestamp of the next mapping is computed as a result.

In practice, the overall schedule is calculated as a sequence of $m$ mappings,
which are dynamically calculated based on the previous mappings results. Thus,
the global schedule may computed recursively using function $Z(m)$ that
utilizes $\vartheta(t)$ defined before to compute every single mapping.  As
shown bellow, the result of each $Z(N)$ is the timestamp of the next
mapping ($N + 1$), which is recursively given as input to $\vartheta(t)$.

\begin{equation}
  Z(m) = \left\{ 
  \begin{array}{l l}
    \beta(0) 		& \quad \text{if $ m = 0$}\\
    \vartheta(Z(m-1))	& \quad \text{otherwise}\\
  \end{array} \right.
%\vartheta(N) = PT_{\phi(\beta(t))} \leftarrow select(T^{\beta(t)}), t'=\beta(t)
\label{eq:mapping2}
\end{equation}

After $m$ mappings, the makespan may be calculated as the $max_{1\le j \le n}
F_j(Z(m))$, or optionally as $max_{1\le j \le n} F_j(\infty)$.  The performance
of the scheduling policies in this framework are differentiated through the
$select$ function implemented by each of them. While FCFS chooses the task with
smallest creation time $c_i \in T^{\beta(t)}$, PRIORITY orders the task in
$T^{\beta(t)}$ according to the expected speedup to select that task with
highest speedups to the GPU and smallest speedup to the CPU. 


==> related.tex <==
\section{Related work} \label{sec:related}
%
The use of hybrid accelerated computing environments is growing in HPC
leadership supercomputing machines~\cite{10.1109/MCSE.2011.83}. The 
appropriate utilization of these hybrid systems,
however, typically requires more complex software instruments to deal with a
number of peculiar aspects of the different processors available.  These
challenging problems motivated a number of languages and runtime
frameworks~\cite{mars,merge,qilin09luk,1616864,Diamos:2008:HEM:1383422.1383447.Harmony,1587427,hpdc10george,6061070,ravi2010compiler,HartleySC10,6152715},
specialize libraries~\cite{opencv_library,icl523}, and compiler
techniques~\cite{1504194,Rudy:2010:PLI:1964536.1964546,5445082}.

Mars~\cite{mars} and Merge~\cite{merge} evaluated the cooperative use of 
CPUs and GPUs to
speedup MapReduce computations. Mars performed an initial evaluation on the 
benefits of partitioning Map and Reduce tasks between CPU and GPU statically. 
Merge extended
that approach with dynamic distribution of work at runtime. 
The Qilin~\cite{qilin09luk} system further proposed an
automated methodology to map computation tasks to CPUs and GPUs. The Qilin strategy
is based on a early profiling phase, where performance data of the target application
is collected, to build a performance model that is used to estimate the best
work division. This approach is able to capture performance variations that
emerge as consequence of input data and application parameters. Unfortunately,
neither of these solutions (Mars, Merge, and Qilin) are able to take advantage
of distributed systems.

Some other projects more recently focused on execution in distributed CPU-GPU
equipped
platforms~\cite{6061070,ravi2010compiler,HartleySC10,6152715,hpdc10george,cluster09george,springerlink:10.1007/s10586-010-0151-6}.
Ravi et al.~\cite{ravi2010compiler,6152715} proposed techniques for automatic
translation of generalized reductions to CPU-GPU environments via compiling
techniques, which are coupled with runtime support to coordinate 
execution. The runtime system techniques introduced a number of auto-tuning
approaches to partition tasks among CPUs and GPUs for generalized reduction
operations. The work developed by Hartley et al.~\cite{HartleySC10} is
contemporary to that of Ravi and proposed similar runtime approaches to
divisible workloads. The work~\cite{6061070} presented DAGuE, a framework to 
enable the use of heterogeneous accelerated machines to executed dense linear 
algebra operations. This system represents the application as a DAG to resolve
dependencies at runtime and, for instance, prioritize the computation of
certain critical paths in the dependency graph in order to maximize
parallelism.

Our work combines the bag-of-tasks pattern with the coarse-grain dataflow 
pattern for efficient execution of scientific data analysis applications. 
Fine-grain 
operations that constitute an analysis pipeline typically involve different 
data access and processing patterns. Consequently,
variability in the amount of GPU acceleration of operations is
likely to exist. This requires the use of performance aware scheduling
techniques in the pipelined computation in order to assign each operation to
the processors it would benefit the most, taking into account the speedups
exhibited by them. In addition, our middleware automatically applies a set of 
optimizations to ensure good performance even in the
case where performance variability is not present or available (i.e., the speedup 
estimates are not computed). The set of optimizations include data locality aware task
assignment, which reduces data movements by taking into consideration the
location where data resides when choosing an operation to execute in a
processors. Data prefetching and asynchronous data transfers are also employed
between CPU and GPU in order to maximizes the GPU utilization, as the data flow
between these devices may occur in parallel to ongoing computation. 





